Phrase-Indexed Question Answering: A New Challenge for Scalable Document Comprehension

We formalize a new modular variant of current question answering tasks by enforcing complete independence of the document encoder from the question encoder. This formulation addresses a key challenge in machine comprehension by requiring a standalone representation of the document discourse. It additionally leads to a significant scalability advantage since the encoding of the answer candidate phrases in the document can be pre-computed and indexed offline for efficient retrieval. We experiment with baseline models for the new task, which achieve a reasonable accuracy but significantly underperform unconstrained QA models. We invite the QA research community to engage in Phrase-Indexed Question Answering (PIQA, pika) for closing the gap. The leaderboard is at: nlp.cs.washington.edu/piqa

==> EMNLP 2018 PIQA/01-intro.tex <==
Extractive question answering (QA) is the task of selecting an answer phrase (span) to a question  given an evidence document.
Due to the easiness of evaluation (compared to generative QA) and the fine-grainess of the answer (compared to sentence-level QA),
it has become one of the most popular QA tasks, driven by
massive new datasets such as \squad~\cite{Rajpurkar2016SQuAD10} and \triviaqa~\cite{joshi2017triviaqa}.
Current QA models heavily rely on  explicitly learning the interaction between the evidence document and the question using neural attention mechanisms ~\citep[\textit{inter alia}]{wang2016machine,xiong2016dynamic,seo2016bidirectional,lee2016learning}, in which the model is fully aware of the question before or as it reads the document.  As a result, despite significant advances, they have not led to the standalone representation of document discourse which is nevertheless a key goal of research in reading comprehension. Furthermore, QA models that condition the document representation on a question have the practical scalability downside that the entire model should be re-applied on the same document for every question. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figures/teaser.pdf}
    \vspace{-.3cm}
    \caption{\qashort\ task for a short context sentence.}
    \label{fig:teaser}
    \vspace{-1mm}
\end{figure}

In this paper, we formalize a modular variant of the QA task, Phrase Indexed Question Answering (\qashort), that enforces complete independence between document encoder and question encoder (Figure~\ref{fig:teaser}).  In \qashort, all documents are processed independently of any question to generate {\it phrase index vectors} (blue nodes in the figure) for each answer candidate (left boxes in the figure).  Similarly, the questions are  independently mapped to {\it query vectors} (red nodes in figure).  Then, at inference time, the answer is obtained by retrieving the nearest indexed phrase vector to the query vector.
Hence the algorithms aimed at tackling  \qashort\  have the inherent benefit of modularity and scalability compared to current QA systems. %\footnote{The \qashort\ task is inherently different from  document or sentence retrieval problems as they achieve {\it content-based} representations, whereas \qashort\ task is based on {\it context-based} representations.}

The task setup is analogous to how documents or sentences are retrieved in modern search engines via similarity search algorithms~\cite{shrivastava2014improved}. Nevertheless, there is a key distinction that search engines index each \emph{document} by its \emph{content}, while \qashort\ requires one to index each \emph{phrase} in documents by its \emph{context}.

We formally define the \qashort\ problem and provide baseline models for the new task. Our experiments show that  the constraint introduced by \qashort\ leads to meaningful standalone document representations and practical scalability advantage, demonstrating the significance of the new task. 
Moreover, there is still a large gap between the baselines and the unconstrained state of the art, showing that the task is yet far from being solved. We have set up a leaderboard\footnote{\web}for \qashort\ challenge and invite the research community to participate. We currently support SQuAD and plan to expand to other datasets as well.
%In Section~\ref{sec:problem}, we first formally define the \qashort\ problem. Then in Section~\ref{sec:baselines}, we discuss baseline models for the new task.
%In Section~\ref{sec:exp}, we experimentally analyze the baseline models and emphasize two key take-aways. First, the constraints introduced by \qashort\ lead to meaningful standalone document representations and practical scalability advantage, demonstrating the significance of the new task. 
%Second, there is still a large gap between the baselines and the unconstrained state of the art, showing that the task is yet far from being solved.

% We hypothesize that \qashort\ requires a stronger model of context-aware phrase representations than the standard QA task, and our experiments with standard methods of document encoding support this hypothesis. An important challenge in \qashort\ is that each phrase is associated with a semantically distinct question according to the context. For instance, in Figure~\ref{fig:teaser}, ``Barack Obama'' can be an answer to two separate questions ``Who is the 44th President of the United States?'' and ``Who was born in 1961?'' We show that defining multiple embedding functions using standard techniques achieves little or no advantage because it requires to compactly diversity those embeddings. 


%Section~\ref{sec:problem} provides the formal definition of the \QA\ problem, and how it relates to phrase representation learning and scalability.
%Section~\ref{sec:baselines} lists competitive baselines using standard techniques in the QA literature. 
%We will see later that, while these models achieve reasonable accuracy, they are far behind the unconstrained state of the art. We make a hypothesis that the major bottleneck comes from the attempt to represent each phrase with a single vector, leading to a conjecture that the phrase representation needs to be \emph{overloaded} with multiple different embedding functions. 


%In particular, we show that an obvious approach of simply defining multiple embedding functions or related techniques borrowed from other domains give little or no advantage, because it is non-trivial to meaningfully and compactly diversify the index vectors.
% In this paper, we propose a novel technique named \emph{pivoting} that uses the surrounding words in the context as pivots to serve as biased priors for context-specific representations of a phrase. 
% For instance, in Figure~\ref{fig:teaser}, ``Barack Obama'' is represented with two index vectors, where the first vector is pivoted with a neighbor word ``President'', whereas the second vector is pivoted with another neighbor word ``1961''.
% The pivot word guides what part of the text the embedding model should focus on, thus giving different foci for different pivots.
% Hence, while two questions ``Who is the 44th President of the United States?'' and ``Who was born in 1961?'' both lead to the same answer ``Barack Obama'', the former question is matched with the first vector while the latter question is matched with the second vector.




% To address this challenge, we present a novel method of \emph{pivoting} to generate multiple diverse encodings of each likely answer candidate. We show that pivoting leads to a 10\% increase in performance on the SQuAD task and we argue for this approach in building phrase representations that are robust across contexts. We also show that our implementation of the PI-QA task has a significant positive impact on scalability since all answer keys can be pre-computed and hashed offline for fast retrieval at query time.



% In short, our contributions are three-fold.
% First, we argue that the independence (modularity) between document encoding and question encoding in QA task is a crucial consideration for advancing research in machine reading comprehension, and it also has a significant implication on the end-to-end scalability of the QA system. We carefully formalize the problem so that it is well-defined and easy-to-evaluate, inviting the research community to easily engage.
% Second, we provide competitive baselines for the new task and analyze them, leading to a conjecture that it is required to have multiple, diverse embeddings for each phrase (answer candidate).
% Third, we propose an effective  technique for diversifying phrase embedding, \emph{pivoting}, that outperforms the baselines by 10\% in Phrase-Indexed SQuAD. In addition, we also present qualitative analysis of the latently learned phrase representations, and discuss the feasibility of extending PI-QA-trained model to a larger-scale QA scenario.



%Recent progress on the task of extractive question answering (QA) with unstructured data such as \squad~\cite{Rajpurkar2016SQuAD10} and \triviaqa~\cite{joshi2017triviaqa} are predominantly based on explicitly learning the interaction between the evidence document and the question using neural attention mechanism ~\citep[\textit{inter alia}]{kadlec2016text}, in which the model is fully aware of the question before or as it reads the document. 
%While it has been an effective strategy, the document encoder can be only defined \emph{with respect to the question}, so it cannot be independently generalized or interpreted (without the question).
%In fact, given that the main purpose of many of these tasks is to evaluate reading comprehension ability, separating the document encoder (comprehension) from the question encoder should be a crucial consideration for the community.
%Furthermore, since the entire model needs to be re-applied on the same document for every new question, modularizing the task is a critical factor for efficiency.

% Toward the goal of modularity and scalability, we propose a new variant of extractive QA task, called \QA\ (\qashort), in which the document and question encoders should be exclusively defined of each other, as shown in Figure~\ref{fig:teaser}.
%  \hh{this is mainly defining your solution than the problem}
%The document encoder first enumerates valid phrases (answer candidates, left boxes in Figure~\ref{fig:teaser}) in the document\footnote{\hh{move this footnote to somewhere in the body of the paper}This is often trivial; enumerating every 7-word or shorter phrase covers 99\% of answers in SQuAD.} and then learns one or more embedding(s) (blue nodes in Figure~\ref{fig:teaser}) for each phrase, which serve as \emph{index} (key) vector(s).
%The question encoder independently maps the question to a query vector (red nodes in Figure~\ref{fig:teaser}).
%Lastly, the predicted answer is obtained by retrieving the nearest index vector to the query vector (dotted lines in Figure~\ref{fig:teaser}).





% After pre-encoding every answer candidate in the corpus of evidence text, \ourapproach\ retrieves answers for new questions by maximizing the inner product between the answer encoding and an analogous question encoding.
% This has the singnificant benefit that answer retrieval can be done via a variant of locality sensitive hashing~\cite{shrivastava2014improved} in sublinear-time with the size of the evidence corpus.
% Hence, \ourapproach\ is the first end-to-end trainable neural question answering model that can scale to large corpora of text at inference time. 
% We call this strategy of learning indexable answer embeddings \emph{context based indexing}.
% This is similar to the \emph{content based indexing} of documents in information retrieval, with the notable exception that we are almost entirely interested in the context \emph{surrounding} an answer candidate, rather than the words that it contains.

% We experiment with \ourapproach\ in \QA\ setup and compare with competitive baselines.
% Specifically, \ourapproach\ has two novel aspects: \textbf{(1)} encoding each answer candidate into multiple contextualized representations rather than into a single embedding. \textbf{(2)} A training-time regularization scheme based on the reconstruction error of generating the question conditioned on the answer. Our experiments show that \ourapproach\  improves over a
% bidirectional LSTM with self-attention baseline by $10\%$ on Stanford Question Answering Dataset via \QA\ (\squad-\qashort). 
% For a scalability test, we also experiment with indexing every answer candidate in the entire \squad\ development corpus, and show that \ourapproach~can retrieve answers from this enormous set both efficiently and with a reasonable degree of accuracy.
% We also present an analysis of phrase representations that \ourapproach\ learns when trained in the \qashort\ setting.

% \todo{Fill in with whatever experiments we have.}
% Since all document interpretation is performed once, prior to execution, we can also constrain our model to only store encodings of likely answer candidate, pivot pairs.
% Doing this, we find that \ourapproach~maintains $xx\%$ of its performance with a $x\times$ reduction in memory. 
% We also examine the pivots and answer boundaries that the model learns to maintain, and find that it learns to identify ?? as useful pivots, and ?? as likely answer boundaries.


% \subsection{Motivation for our Approach}

% Before giving a technical description of our model, we first consider an example for motivation. Consider Figure~\ref{fig:teaser} where two questions $Q$ and $Q'$ are presented, both where the correct answer is \textit{Barack Obama}. In the text, there are multiple facts about \textit{Barack Obama} presented, specifically that he was the 44th president and that he was inaugurated in 2009 (Other documents could discuss his family or political views).

% A first strategy would be to encode all this information into a single vector. However, this makes it difficult to discern whether \textit{Barack Obama} is an answer to a particular question that may depend on only one of these facts. For instance $Q'$ is only asking about the \textit{44'th president} and the inauguration date is irrelevant to answering the question.

% Instead, we propose to associate each answer candidate with multiple vectors, each created with respect to a different \textit{pivot}. In Figure~\ref{fig:teaser} these two pivots are \texitit{44'th} and \textit{2009}. Analogously, questions can also be encoded with respect to different triggers (\texitit{44'th} and \textit{2010} in this case). Given a question-trigger vector, our model then finds the answer candidate-pivot pair with the largest maximum inner product.



%\textit{Barack Obama}







% we introduce an end-to-end trainable method of 
% Prior to execution, \ourapproach~precomputes an encoding of all answer candidates.
% At execution time \ourapproach~then encodes the question into the same space and performs nearest-neighbor search among the precomputed candidate encodings to select an answer.
% Question, answer-candidate compatibility is defined as the euclidean distance between their encoding vectors.
% Since this metric supports sub-linear nearest neighbor search \cite{}, \ourapproach~is the first end-to-end trainable deep learning system for extractive question answering. 


%In addition, we also argue that it is an important extension of current reading comprehension tasks, since it introduces the requirement that our models must learn which parts of the document are important in general, not just in the context of a specific question.






%Since this approach does not scale to arbitrarily long evidence texts, recent work has proposed a pipelined approach that first uses traditional information retrieval (IR) techniques to deterministically \tk{Is this actually true???} sample a small set of candidate sub-texts that for which a question-dependent representation can be built.

%While these pipelined approaches do scale to large evidence corpora, they still require an expensive joint encoder to be run on multiple paragraphs every time a new question is seen.
%Even with the most powerful off-the-shelf computational resources available today, these models take ?? \todo{Numbers from Minjoon's slides} GPU seconds or ?? CPU seconds per paragraph.
%They are subsequently not viable candidates for real-world question answering systems.
%Furthermore, since they are not end-to-end trainable, pipelined approaches are upper bounded by the accuracy of an IR system that was designed for document retrieval, not question answering.


% In this paper we introduce, for the first time,  question-independent document encodings for extractive question answering. \ourapproach takes advantage of a novel neighbor word pivoting mechanism to encode information about all of the answer candidates and all of the questions that could be asked of them. \hh{we can refer to the teaser figure/obama example}
% Additionally, \ourapproach leverages a novel dual learning objective to address xxx. 


%We show that a vanilla bidirectional LSTM document encoder is not effective and we hypothesize that this is for two reasons. 
%First, without access to question-dependent attention weights, the LSTM cannot sufficiently encode information about all of the answer candidates and all of the questions that could be asked of them.
%Second, the purely linear interaction between question and document encodings hinders learning \todo{Citation}. 
%In \sect{sec:pivot} we introduce a novel neighbor word pivoting mechanism to deal with the first of these issues and in \sect{sec:dual} we introduce a dual learning objective to deal with the second.
%With both of these modifications we improve performance on the \squad~task by $10\%$.

%While the performance of \ourapproach~is well behind the current state-of-the art on \squad, it performs similarly to equally simple architectures that topped the leaderboard one year ago.



==> EMNLP 2018 PIQA/02-related.tex <==
\vspace{-.2cm}
\paragraph{Reading comprehension.}
Massive reading comprehension question answering datasets~\cite{hermann2015teaching, hill2015goldilocks, dhingra2017quasar, dunn2017searchqa} have driven a large number of successful neural approaches~\citep[\textit{inter alia}]{kadlec2016text,hu2017reinforced}.  
% The community has also moved beyond paragraph-size documents to larger documents and multiple web results~\cite{dhingra2017quasar,dunn2017searchqa,joshi2017triviaqa}.
~\citet{choi2017coarse,chen2017reading,clark2017simple,min2018efficient} tackled large-scale QA by using a fast, coarse model (e.g. TF-IDF) to retrieve few documents or sentences and then using a slower, accurate model to obtain the answer.
% One disadvantage of such pipeline is that the fast and slow models are independently learned. \citet{nogueira2017task,swayamdipta2017multi} address this issue via reinforcement learning or cascade.
\citet{salant2017contextualized} proposed to minimize (but not prohibit) the influence of question when modeling the document.
Similarly to ours, \citet{lee2016learning} proposed to explicitly learn the representation for each answer candidate (phrase) in the document, but it was conditioned (dependent) on the question.

% All of these architectures heavily depend on attention mechanism to encode the document with respect to the question and thus do not yield standalone document representation models.


% Thus, to our knowledge, our approach is the first to be capable of running an end-to-end neural QA model at inference time over a massive corpus with sublinear time complexity.

\vspace{-.2cm}
\paragraph{Sentence retrieval.} A closely related task to ours is that of retrieving a sentence/paragraph in a corpus that answers the question~\citep{tay2017hyperqa}. A comprehensive survey for neural approaches in information retrieval literature is discussed in~\citet{mitra2017neural}. 
We note that our problem is focused on phrasal answer extraction, which presents a unique challenge over sentence retrieval---the need for \textit{context-based} representation as opposed to the \textit{content-based} representation in the sentence-retrieval literature.

%QA in IR. These are at finest sentence-level and not word level. Talk about transfer learning, and why word-level is essential for sentence level as well. ~\cite{hyperbolic} Neural IR




%mitra2017neural
\vspace{-.2cm}
\paragraph{Language representation.} Recently there has been a growing interest in developing natural language representations that can be transferred across tasks~\citep[\textit{inter alia}]{vendrov2015order,wieting2015towards, conneau2017supervised}.
In particular, SNLI~\cite{SNLI} and MultiNLI~\cite{williams2017broad} encourage architectures that first encode the hypothesis and the premise independently before a comparator neural network is applied.
Our proposed problem shares similar traits but has a stronger constraint that only inner product comparison is allowed and one needs to model phrases instead of complete sentences.

%SNLI~\cite{SNLI}, sentence rep, etc. MultiNLI~\cite{williams2017broad}
%. While not the focus of this work, our formulation could also help advance phrase 


% Ankur: I think related work on question generation / multi-sense embeddings can be discussed in the corresponding model section.
% One key te is related to work e.g. ~\cite{lin2017structured} where the goal is to create multiple embeddings for each word. 

% \paragraph{Multi-Sense Embedding.} Also talk about diversifying representation by sampling from prior distribution. 

% \paragraph{Question Generation.} For dual learning.~\cite{tang2017question,duan2017question,yuan2017machine}

% \paragraph{Similarity Search.} NNS, MIPS, their speed, etc.

\paragraph{Memory networks.} Each phrase-vector is analogous to a single memory slot, where the vector is the key and the phrase is the value, and the question vector is the query for accessing the memory. Hence, \qashort\ can be considered as an effort to formulate extractive question answering as the task of memory augmentation (construction)~\cite{memory, sukhbaatar2015end} from unstructured knowledge source (text).

==> EMNLP 2018 PIQA/03-problem.tex <==
Extractive question answering is the task of obtaining the answer $\hat a$ to a question $Q = \{q_1 \dots q_n\}$ given an evidence document $D = \{ d_1 \dots d_m \}$, where the answer $\hat a = (s, e)$ indicates the start and end of a span in the document.
The task is often formulated as learning the probabilistic distribution of the answer given the question and the document. 
In existing literature (\sect{sec:related}), the distribution is mainly featurized by $\paramp(a|Q,D) \propto \exp(\complexqa(Q, D, a))$ where $\complexqa$ could be any real-valued scoring function parameterized by $\theta$.
Once $\theta$ is learned, the prediction $\hat{a}$ is obtained by
\begin{equation}
\hat a = \argmax_{a} \complexqa(Q, D, a).
\end{equation}
% $\complexqa$ can be also \emph{overloaded} with several different functions and then aggregated via $\argmax$, which corresponds to how most ensemble methods work.
So far, most competitive designs of $\complexqa(Q,D,a)$ make use of attention connections between the words in $Q$ and $D$.
As a result, these models cannot yield a query independent representation of the document $D$. It is subsequently not possible to independently assess the document understanding capability of the model. Furthermore, $\complexqa(Q, D, a)$ needs to be re-computed for the entire document for every new question. We believe that this inefficiency  precludes all current models as the candidates for end-to-end QA systems.

We propose a new task---\QA\ (\qashort)---that addresses these issues. 
We enforce the \emph{decomposability} of $\complexqa$ into two exclusive functions $\encq(Q), \encd(D, a) \in \mathbb{R}^k$. 
The answer distribution is then modeled by $\paramp(a|Q,D) \propto \exp(\encq(Q) \bullet \encd(D, a))$, where $\bullet$ is the inner product. The prediction is obtained by 
\vspace{-0.5mm}
\begin{equation}
  \hat a = \argmax_{a} \encq(Q) \bullet \encd(D, a).
  \label{eqn:form2}
\end{equation}
% Similarly to Equation~\ref{eqn:form1}, $\encq$ and $\encd$ can be also overloaded.
% Furthermore, $\encd$ now only needs to be computed once per document regardless of the number of questions.
In this setting, the document encoder $\encd$ learns models the document independently of the question.
Successful question answering models that follow the structure of \qashort\ will have two important advantages over current QA models: full document comprehension and scalablity. 

\paragraph{Full document comprehension.}  Language understanding ability is widely associated with learning a good standalone representation of text (or its components such as phrases) independent of the end task~\cite{SNLI}. Under \qashort\ constraints, the document encoder $\encd$ learns the representation of the answer candidate phrases $a$ in the document $D$ independent of the question. In order to correctly answer questions, these  phrase representations (index vectors) need to correctly encode their meaning with respect to their context. 
Therefore,  \qashort\ constraint enforces evaluating research in document comprehension and phrase representation learning.%\footnote{Phrase representations can be further enhanced with document- (or paragraph-) level representations, such as tf-idf vectors, which recently have been shown to be effective for large-scale question answering~\cite{chen2017reading,clark2017simple}.
% Unlike the previous work, where the tf-idf-based search had to be pipelined, \qashort\ allows end-to-end search in a single shot via simple concatenation of the tf-idf vectors and the phrase vectors.
% }

% $\encq$ is the question encoder that maps the question to a query vector in the same vector space. Answering is simply done by finding the argmax of the inner product between the query vector and the index vectors. \hh{add a sentence why this is comprehension}


\paragraph{Scalability.} Models that adhere to the \qashort\ constraint only need to be run once for each document, regardless of the number of questions asked. 
To answer a question, the model then just needs to encode the question and compare it to each of the answer candidates via the inner product in Equation~\ref{eqn:form2}.
Implemented naively, computing a single inner product for each answer candidate is more efficient than building a new document encoding; after the documents are pre-encoded, Equation~\ref{eqn:form2} is $O(k)$ time per word where $k$ is the vector size (most neural models require $O(k^2)$ per word for matrix multiplications).
%\footnote{Let $n$ be the total number of $(D, a)$ pairs. Then the computational complexity of solving Equation~\ref{eqn:form2} is computing $n$ inner products in $d$-dimensional vector space, $O(nd)$.
% Since most neural QA architectures (that follows Equation~\ref{eqn:form1}) require matrix computations (mostly for RNNs and attention), which is $O(d^2)$ the final time complexity is $O(nd^2)$. Hence \QA\ has a definite computational advantage over unconstrained QA systems.}

% lead to designing question answering models that can be applied in a large collection of documents. \hanna{Min, is this correct?} An obvious benefit is that $\encd$ needs to be computed only once per document.
% This becomes computationally effective as soon as more than one question is asked of each document---a
% We now discuss how the imposed constraint in \QA\ problem enables efficient answer retrieval, even for an extremely large corpus.
% We rewrite Equation~\ref{eqn:max-piv} in two stages:
% \begin{align}
% \hat{a} & = \argmax_{a, \trigger \in \triggerfeat(Q)} \qb_{\trigger}^\top \hat{\ab}^{\trigger} \textrm {\,\,where } \label{eq:mips-final} \\
% \hat{\ab}^{\trigger} & := \argmax_{\tilde \ab_{\pivot} \, \forall \pivot \in \pivotfeat(D, a)}  \tilde \qb_{\trigger}^\top \tilde \ab_{\pivot}
% \label{eq:mips-sub}
% \end{align}
% where first for each $\trigger \in \triggerfeat(Q)$, we find the answer with the highest inner product. We then take the maximum over all the possible $\trigger$.
% First consider the inference complexity of the exact solution at query time.
% Since the document encoder $\encd$ doesn't depend on the question, it can be precomputed for all $(D, a)$ pairs. We also consider the computational cost of the question encoder $\encq$ to be negligible since questions are usually only a few words. 

More importantly, 
%A less obvious but more important benefit is that the formulation 
\qashort\ also permits an approximate solution in sublinear time using asymmetric locality-sensitive hashing (aLSH)~\cite{shrivastava2014asymmetric, shrivastava2014improved},
% . Under aLSH, 
%query and answer vectors are hashed into the same bin  vector will be hashed into the same bin that contains the closest answer vector if and only if the inner product is greater than a given threshold.
through which Equation~\ref{eqn:form2} can be approximated for $N$ answer candidates with $O(k N^\rho  \log N)$ time, where $\rho < 1$ is a function of the approximation factor and the properties of the hash functions.
We argue that this type of approach will be essential for the development of real world QA systems, where the number of potential answers $N$ is extremely large.

%  In particular, the formulation can take the full advantage of maximum inner product search (MIPS) algorithms when $n$ becomes extremely large (i.e. very large corpus of documents). More concretely,
% In practice, for large-scale question answering, as we showed in ``Scalability'' part of Section~\ref{sec:problem}, we will need to concatenate the phrase embedding with document embedding (e.g. TF-IDF-based vector), since the phrase embedding is learned conditioned on the document, not the entire corpus. Still, it is easy to see that the concatenated embedding will enjoy a similar computational advantage. 
% Also, while we discussed the general case of \qashort\, note that a similar conclusion can be drawn for the pivoted encoders as well.

% The probability of the correct answer $a$ to the question $Q$ for a large corpus of documents $C=\{D_1, \dots D_L\}$ can be computed as $\paramp(a|Q,C) = \sum_i \paramp(a,D_i|Q,C) = \paramp(a,D^a|Q,C)$ where $D^a$ is the document that contains the span $a$ (every other document should give zero joint probability).
% Assuming independence among documents, chain rule gives us $\paramp(a,D^a|Q,C) = \paramp(a|Q,D^a) \paramp(D^a|Q,C)$, where $\paramp(a|Q,D_i)$ is the question answering model, and  $\paramp(D_i|Q,C)$ is a document retrieval model.
% If we let $\paramp(D_i|Q,C) \propto \exp(\encq^C(Q) \bullet \encd^C(C,D_i))$, where $\encd^C$ is a document embedding function (e.g. tf-idf) and  $\encq^C$ is a corresponding question embedding function dedicated for document retrieval, then the final prediction is
% \begin{equation}
% \begin{split}
%   \hat a = \argmax_{a,i} & [\encq(Q),\encq^C(Q)] \\
%    & \bullet [\encd(D_i, a),\encd^C(C,D_i)]
% \end{split}
% \end{equation}
% where $[,]$ is vector concatenation.
% MIPS algorithms can index (hash) the concatenated vectors $[\encd(D_i, a),\encd^C(C,D_i)]$ offline so that the best answer can be found at query-time efficiently.
% While web-scale question answering is out of the scope of this paper, it is worthwhile noting that this formulation allows a homogeneous joint model even for an extremely large scale corpus, in contrast to pipelined methods such as DrQA~\cite{chen2017reading} whose question answering model cannot influence the outcome of the document retrieval model\footnote{As noted, QA will be less accurate and overall performance might be lower. An important research challenge would be whether we can close the gap and outperform the pipelined method.}. 
% Also note that the chain rule can be used for an arbitrary number of layers; for instance, one can have three layers (paragraph-document-corpus) instead of two layers (document-corpus).

% Extractive question answering is the task of obtaining the answer $\hat a$ to a question $Q$ given an evidence document $D$.  In existing literature (``Reading comprehension'' in \sect{sec:related}) single-answer extractive question answering is formulated as learning a prediction function $\complexqa(Q, D, a)$ such that 
% \begin{equation}
%   \hat a = \argmax_{a} \complexqa(Q, D, a)
%   \label{eqn:form1}
% \end{equation}
% Where $\hat a = (i, j)$ is the index pair that delimits the span of text in the corpus $D = \{d_0, \dots, d_m\}$ that answers the question $Q = \{q_0, \dots, q_n\}$, where $d_i$ and $q_i$ are words.
% Typically, $\complexqa$ is a neural network that interleaves LSTM encoders with attention mechanisms that take both $Q$ and $D$ as input.

% In this paper we reformulate the extractive question answering to require the document be encoded agnostic of the question.  Specifically, we examine prediction functions of the form
% \begin{equation}
%   \hat a = \argmax_{a} \encq(Q)^\top\encd(D, a)
%   \label{eqn:form2}
% \end{equation}
% where $\encq(Q) \in \RR^d$ and $\encd(D, a) \in \RR^d$ are functions that map the question and the answer candidate into a $d$ dimensional vector space.
% Equation \ref{eqn:form2} poses a significantly stronger constraint than the general form in Equation \ref{eqn:form1} due to the impoverished interaction between $Q$ and $D$.
% However, it does have the significant advantage that $\encd(D, a)$ can be run prior to inference to encode all answer candidates.
% Now, when a new question is seen, we only need to run $\encq(Q)$ and use a maximum inner-product search algorithm\footnote{A similar argument can be made for other sublinear search algorithms (e.g. L1, L2, or cosine distance).} to get the best answer.
% In \sect{sec:nn-search} we explain how this results in an execution time that is sublinear in the size of the evidence corpus.
% In \sect{sec:sublin-exp} we show how our model can scale in practice, allowing us to ask questions of several orders of magnitude more text than existing neural methods.


% ------ OLD TEXT ------- % 

% Text-based question answering is the task of obtaining the answer to a question given contextual text.
% We let ${\bf C} \in \mathbb{R}^{C \times E}$ represent the embedded context words, where $C$ is the number of context words and $E$ is the embedding size.
% Similarly, we let ${\bf Q} \in \mathbb{R}^{Q \times E}$ represent the embedded question words, where $Q$ is the number of question words.
% We let ${\bf V} \in \mathbb{R}^{V \times E}$ represent the vocabulary embedding, where $V$ is the vocabulary's size.
% Let ${\bm a}$ be the representation for a candidate answer phrase, which is often defined as a pair of start and end position of the phrase in the context, i.e. ${\bm a} = (a_\mathrm{start}, a_\mathrm{end})$.
% Our objective is to find
% $\hat{\bm a} = \arg \max_{{\bm a}} \mathrm{Pr}({\bm a}|{\bf Q}, {\bf C})$.
% In question answering literature, the task is often formulated as learning a scalar function $k$ that scores the likelihood of the answer candidate with respect to the context and question\footnote{In the case of extractive question answering, number of answer candidates is strictly linear in the size of context, thus it is indeed tractable to enumerate them and score each of them.}: 
% \begin{equation}
% \mathrm{Pr}({\bm a}|{\bf Q}, {\bf C}) \propto \exp(k({\bf Q}, {\bf C}, {\bm a})),
% \end{equation}
% which leads to $\hat{\bm a} = \arg \max_{\bm a} k({\bf Q}, {\bf C}, {\bm a})$.
% Such formulation allows powerful modeling of interaction between the context and question, such as (cross) attention mechanism.
% However, the biggest drawback of this formulation is that for every new question, the function needs to be applied to the entire context, which often means the computational cost is linear in the size of the context.
% To resolve this issue, we impose a strong restriction on $k$ by {\bf featurization}\footnote{This is analogous to the inverse of kernelization (for kernel method), where $k$ is analogous to the kernel function.}:
% \begin{equation}\label{eqn:feature}
%     k({\bf Q}, {\bf C}, {\bm a}) = -d({\bm \uppsi}({\bf Q}), {\bm \upphi}({\bf C}, {\bm a}))
% \end{equation}
% where ${\bm \uppsi}$ and ${\bm \upphi}$ are feature functions to be learned and $d()$ is a metric (Euclidean distance function).
% Hence $\hat{\bm a} = \arg \min_{\bm a} d({\bm \uppsi}({\bf Q}), {\bm \upphi}({\bm a}, {\bf C}))$, i.e. finding the nearest neighbor.
% Note that now the context and the question can only interact through the distance function, hence more challenging problem than learning $k$ without any restriction.
% Nevertheless, featurization has three crucial advantages.
% First, ${\bm \upphi}$ only needs to be computed once and can be precomputed.
% Second, finding the argmax of Equation~\ref{eqn:feature} can be approximated with nearest neighbor search in sublinear-time (practically constant-time) by locality-sensitive hashing (LSH) of ${\bm \upphi}$.
% This means that for real-time question answering scenario, once preprocessing of context is completed, it only needs to compute ${\bm \uppsi}({\bf Q})$, which is then used to find the best answer in the hash table.
% Lastly, by allowing interaction only via distance function, ${\bm \upphi}$ is forced to be feature-rich representation of the (answer) phrase. This is well-aligned with recent effort on language inference task~\cite{SNLI} where premise representation and hypothesis representation are independently obtained and only shallow neural network is allowed on top of them to obtain the final classification prediction. 

% An important intuition through out this paper is that, if ${\bm \uppsi}$ is close to an isomorphism (i.e. a good representation function of the question), learning ${\bm \upphi}$ is roughly equivalent to the task of predicting what question can be asked (i.e. question generation) for the given context and the answer candidate  in vector space. 
% Hence, while technically not a generative model (of language), we conjecture that ${\bm \upphi}$ shares many characteristics with generative model, which will be useful to motivate our models in Section~\ref{sec:model} and explain results in Section~\ref{sec:exp}. 

==> EMNLP 2018 PIQA/04-baselines.tex <==
% Since \qashort\ is significantly more constrained than existing QA tasks, 
We introduce several baselines for \qashort\ that are motivated by related literature.
% We will then discuss the limitations of this model, and we introduce a novel model architecture designed to deal with these in Section~\ref{sec:pivoting}.
%due to the imposed structural constraint, we 
% We also discuss the limitation of these standard techniques for \qashort\, which will lead to our proposed model that addresses them in Section~\ref{sec:pivoting}.

For all (neural) baselines, we represent the words in $D$ and $Q$ with one of three embedding mechanisms:
CharCNN~\cite{kim2014convolutional} + GloVe~\cite{pennington2014glove}, and ELMo~\cite{peters2018deep}.
We follow the majority of the related literature and apply bidirectional LSTMs~\cite{Hochreiter:97} to these embeddings to build the context-aware representations of the document ${\bf D} = \{{\bf d}_1 \dots {\bf d}_m\}$ and question ${\bf Q} = \{{\bf q}_1\dots {\bf q}_n\}$, where the forward \& backward LSTM outputs are concatenated to get a single word representation, i.e. ${\bf d}_i, {\bf q}_i \in \mathbb{R}^{2k}$ where $k$ is the hidden state size of LSTMs.
% Done! % \paragraph{Self-attention.} 

\qashort\ disallows cross-attention between document and question.
However, we can still benefit from self-attention, which has become crucial for machine translation~\cite{vaswani2017attention} and QA~\cite{huang2017fusionnet, wei2018fast}.
In all of our baselines, each variable-length question is collapsed into a fixed length vector via the sum 
 ${\bf q}^\text{SA} = \sum_i u_i {\bf q}_i$ where ${\bf u} = \{u_1\dots u_n\}$ is a vector containing a single weight for each word in the question. 
Similarly, we experiment with document side self attention to represent each document word ${\bf d}_j$ as a weighted sum of itself and all neighboring words ${\bf d}^\text{SA}_j = \sum_i h^j_i {\bf d}_j$.
The weight vectors $\bf u$ and ${\bf h}^j$ are calculated as
\begin{align}
    {\bf u} &= \mathrm{softmax}_i({\bf w}^\top {\bf q}_i) \notag \\ 
    {\bf h}^j &= \mathrm{softmax}_i(R_{\theta}({\bf D}, j)^\top K_{\theta}({\bf D}, i)) \notag
\end{align}
%where ${\bf u}$ contains a weight for each of the words in the question and ${\bf h}^j$ weights each of the words in the document in the context of the word at position $j$.
where $R_\theta$, and $K_\theta$ are trainable neural networks with the same ouptut size, and ${\bf w} \in \mathbb{R}^{2k}$ is a trainable weight vector.
We use independent BiLSTMs with hidden state size $k$ (i.e. the output size is $2k$) to model both $R_\theta$ and $K_\theta$. That is, $R_\theta({\bf D}, j)$ is the $j$-th output of BiLSTM on top of ${\bf D}$, and we similarly define $K_\theta$ with unshared parameters.


For all (neural) baselines, the question is represented using the concatenation of two copies of ${\bf q}^\text{SA}$, one that should have high inner product with the vector for the answer's start span and another that should have high inner product with the vector for the answer's end. Thus, Equation~\ref{eqn:form2}'s $\encq(Q)=[{\bf q}^\text{SA}_{s}, {\bf q}^\text{SA}_{e}]$ where the subscripts $s$ (start) and $e$ (end) imply that different sets of parameters were used.
Now we define several baselines.

\paragraph{LSTM baseline.}
An answer candidate $a = (s,e)$ is represented using the LSTM outputs at its endpoints: from Equation~\ref{eqn:form2}, $\encd(D,(s,e)) = [{\bf d}_s, {\bf d}_e] \in \mathbb{R}^{4k}$ and $\encq(Q)=[{\bf q}^\text{SA}_{s}, {\bf q}^\text{SA}_{e}] \in \mathbb{R}^{4k}$.

\paragraph{LSTM+SA baseline.}
The LSTM outputs are augmented with the endpoint representations that come out of the document's self-attention (SA):
$\encd(D,(s,e)) = [{\bf d}_s, {\bf d}^\text{SA}_s, {\bf d}_e, {\bf d}^\text{SA}_e] \in \mathbb{R}^{8k}$ and $\encq(Q)=[{\bf q}^\text{SA}_{s1},{\bf q}^\text{SA}_{s2}, {\bf q}^\text{SA}_{e1},{\bf q}^\text{SA}_{e2}] \in \mathbb{R}^{8k}$.

% \paragraph{PE+SA baseline} 
% This baseline follows~\cite{vaswani2017attention} in using a sinusoidal position encoder (PE) instead of an LSTM to encode words in position. Otherwise, the self-attention mechanism is the same as in LSTM+SA.


%With these weights, we create a vector representation of the query ${\bf q}^\text{SA} = \sum_i {\bf u}_i {\bf q}^\text{L}_i$, and a self-attention augmented representation of the $j$-th document word ${\bf d}^\text{SA}_j = \sum_i {\bf h}^j_i {\bf d}^\text{L}_j$.
%We then represent each answer candidate $a = (s, e)$  as $\encd(D,(s,e)) = [{\bf d}^\text{SA}_s, {\bf d}^\text{SA}_e]$ and let $\encq(Q)=[{\bf q}^\text{SA}_s, {\bf q}^\text{SA}_e]$ (we loosely use subscripts $s,e$ to indicate that we use different trainable weights for start and end).

%In practice, it is more beneficial to have multiple heads (instead of single head) of the attention.
%That is, we can compute multiple weight vectors ${\bf u}_1 \dots {\bf u}_N$, where $N$ is the number of heads, and concatenate the attended vectors to obtain $\encq(Q)$ (and obtain $\encd(D, (s,e))$ in a similar way).
%In our experiments, we use two heads, where one of the attention is identity attention on the document side (i.e. ${\bf d}^\text{SA}_j = {\bf d}^\text{L}_j$).

%\tk{I would cut this paragraph if we need the space. I don't think it adds much, and you do not discuss the results.}
%Note that the self-attention models originally use a sinusoidal position encoder (PE) instead of LSTM for parallelization and thus speed up at little cost of drop in accuracy, which we include in our baseline results.
%We also experiment with a simpler baseline where we use LSTM outputs instead of the attention vectors, i.e. $\encd(D,(s,e)) = [{\bf d}^\text{L}_s, {\bf d}^\text{L}_e]$. In this case, we only use a single head (not multi-headed).
\paragraph{TF-IDF.} We lastly include a purely TF-IDF-based model, where each answer candidate phrase is associated with a bag of neighbor words within a distance of 7. Then the BOW vector is normalized via TF-IDF and indexed. When the query comes in, its TF-IDF vector is queried on the indexed phrases to yield the answer.

\paragraph{}For training the (neural) models, we minimize the negative log probability of getting the correct answer: the loss function for each example $(D, Q, a^*)$ is $L(\theta) = -\log \paramp(a^*|D,Q)$ where $a^*$ is the correct answer.

% ${\bf w} \in \mathbb{R}^d$ is a trainable weight vector and $K^\text{Q}_\theta$ is a trainable neural network of output size $d$.
% Then we obtain the query vector by $\encq(Q) = \sum_i {\bf w}_i {\bf q}^\text{L}_i$.

% On document encoding side, we obtain the attention weight vector for each $j$-th word by ${\bf h}^j = \mathrm{softmax}_i(R_\theta({\bf d}^\text{L}_j) K_\theta^\text{D}({\bf d}^\text{L}_i))$, where $R_\theta, K_\theta^\text{D}$ are trainable neural networks of output size $d$. Then similarly each attention vector is obtained by ${\bf d}^\text{SA}_j = \sum_i {\bf h}^j_i {\bf d}^\text{L}_j$.
% Finally, to obtain the phrase representation, we concatenate the self-attended document vector of the start and the end positions: $\encd(D,(s,e)) = [{\bf d}^\text{SA}_s, {\bf d}^\text{SA}_e]$.

% TOM: I'm moving some of this argument in to the next section. It's a bit weird here and we can talk about the baseline with 
%   multiple representations by just saying it's equivalent to a single pivot value being sampled k times.  

% \paragraph{Overloading.} As we will see in Section~\ref{sec:exp}, while the above baseline model gives a reasonable accuracy in \qashort\, it substantially underperforms the state of the art without the constraint.
% One of the main limitations is that the document encoder $\encd$ only gives a single embedding for each answer candidate phrase.
% Referring to Figure~\ref{fig:teaser} again, recall that two semantically different questions should be allowed to map to the same answer.
% \emph{Overloading} $\encd$ lets us to generate multiple embeddings for each phrase, each of which can be associated with a semantically different question.
% An obvious, trival way to overload the encoder is to make $n$ copies of the encoder, each of which having independent weights, and aggregate them later with $\max$.
% Nevertheless, as we will see, this does not diversify the phrase embeddings, which does not provide any advantage over the vanilla baseline. 
% Hence a unique challenge to \qashort\ is to design an effective overloading mechanism that can generate multiple interesting and different representations of each phrase, which will be the main focus of Section~\ref{sec:pivoting}.


==> EMNLP 2018 PIQA/05-exp.tex <==
%The experimental section serves three purposes. 
% First, we report the accuracy of the baseline models for \qashort, showing that they achieve reasonable accuracy while falling short of the state of the art in the standard (unconstrained) setting.
% Second, we analyze the  phrase representations learned by the document encoder that capture lexical and syntactic information.
% Third, we discuss the scalability advantage of the paradigm, which offers several orders of magnitude faster inference with manageable memory cost.
\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{clcc}
        \toprule
        Constraint & Model & F1 (\%) & EM (\%) \\
        \midrule
        \multirow{ 5}{*}{PI} & TF-IDF & 15.0 & 3.9\\
         \cline{2-4}
         & LSTM & 57.2 & 46.8\\
         & LSTM+SA & 59.8 & 49.0\\
         \cline{2-4}
         & LSTM+ELMo & 60.9 & 50.9\\
         & LSTM+SA+ELMo & 62.7 & 52.7\\
         % LSTM+SA+Emb+Gen & 65.1 & 54.2\\

		\midrule
        \multirow{2}{*}{None}  & \citet{Rajpurkar2016SQuAD10} & 51.0 & 40.0\\ 
         & \citet{wei2018fast} & 89.3 & 82.5\\
        % \midrule
        % \ourapproach--RR  & 67.9 & 57.2\\
        % \ourapproach--Piv & 62.3 & 51.5\\
        % \midrule
        % \ourapproach--Att & 68.3 & 57.8\\
        % \ourapproach--Att--RR & 68.0 & 57.2 \\
        % \ourapproach--Att--Piv & 58.4 & 48.1 \\
        \bottomrule 
    \end{tabular}
    }
    \caption{Performance on \squad\ dev set with the \qashort\ constraint (top), and without the constraint (bottom). See Section~\ref{sec:baselines} for the description of the terms.}
    \label{tab:squad}
\end{table}

% \paragraph{Dataset \& setup.} 
We impose the independence restrictions from \qashort\ on the Stanford Question Answering Dataset\footnote{PIQA paradigm can be also extended to other extractive QA datasets.}. 
%We will use ``PI-SQuAD'' to specifically refer to the task. 
We only consider answer spans with  length $\leq 7$. We use the hidden state size ($k$) of $128$, which results in a 512D ($4k$) and 1024D ($8k$) vector for each phrase in LSTM and LSTM+SA, respectively. The default embedding model is CharCNN concatenated with 200D GloVe, with an option to append ELMo vectors following the same setup for SQuAD experiments discussed in~\citet{peters2018deep}. We use a batch size of $64$ and train for $20$ epochs with the default Adam optimizer~\cite{adam}, and take the best model on the validation set during training.

\paragraph{Results.}
Table~\ref{tab:squad} shows the results for the \qashort\ baselines (top) and the unconstrained state of the art (bottom). % `PE' refers to Position Encoder, `SA' refers to Self-Attention, 
%`ELMo` indicates that word representations were built using ELMs, `Emb' indicates that only the word embeddings were taken from that model. `Ens' refers to an ensemble, and `Reg' refers to the multi-sense embedding regularization by~\citet{lin2017structured}.
First, the TF-IDF model performs poorly, which signifies the limitations of traditional document retrieval models for the task.
Second, we note that the addition of self-attention makes a significant impact on results, improving F1 by 2.6\%. 
% has  LSTM+SA is better than using LSTM alone or replacing LSTM with PE.
Next, we see that adding ELMo gives 3.7\% and 2.9\% improvement on F1 for LSTM and LSTM+SA models, respectively.
Lastly, the best \qashort\ baseline model is 11.7\% higher than the first (unconstrained) baseline model~\citep{Rajpurkar2016SQuAD10} and 26.6\% lower than the state of the art~\citep{wei2018fast}.
This gives us a reasonable starting point of the new task and a significant gap to close for future work.
% First, the baseline LSTM model does manage to predict just under half of the answers exactly, which is 8\% better than the original baseline~\citet{Rajpurkar2016SQuAD10}. Adding self-attention (SA) above the LSTM gives a non-trivial boost.
% There is still a clear gap between the baseline models and the state of the art, due to the PI-constraint.



% Adding self-attention to the LSTM improves performance significantly, since the answer candidate representation now has direct access to distant context. 
% However, as we mentioned in \sect{sec:reg-rec}, we observed that the model resulted in high generalization error (i.e. overfitted). 

% \ourapproach~ significantly outperforms the two baselines\footnote{We have recently submitted our model to the leaderboard to be evaluated on the hidden test set, and will be available soon anonymously on \url{http://stanford-qa.com}}. While the performance of \ourapproach~is  behind the current state-of-the art on \squad, we  emphasize that the \qashort\ formulation is inherently different and much more restrictive than the standard QA task on SQuAD. It is interesting to observe that \ourapproach~ performs similarly to architectures that topped the leaderboard one year ago.

% \paragraph{Ablations.} We study the effect of ablating different components of our model, namely pivoting, reconstruction loss, and self attention. Removing the regularization through reconstruction loss (shown in \ourapproach--RR and \ourapproach--Att--RR )  hurts the performance, but it makes a greater impact on the model with self-attention; \ourapproach--Att--RR only loses 0.3\% from \ourapproach--Att, while \ourapproach--RR loses 1.7\% from \ourapproach. As we described in \sect{sec:reg-rec}, we conjecture that this is due to higher overfitting capability of LSTM+Att.

% Finally, our key contribution---pivoting---improve performance across the board. The table shows that removing the pivoting drops the performance significantly (shown by comparing \ourapproach--P and \ourapproach--Att--P). 
% The results in Table~\ref{tab:squad} use the word indicator pivot features from \sect{sec:pivot-feat} with the $\alpha$ and $\gamma$ that are high enough so that it forces a (trigger, pivot) match if one is available.
% We also experimented with the dense embedding features introduced in \sect{sec:pivoting} but found that these gave slightly worse overall performance ($67.5\%$ F1, $57.0\%$ EM).
% We believe that this may be an artifact of the \squad, which has a high degree of word overlap between question and context~\cite{jia2017adversarial}, and we intend to explore more robust trigger and pivot combinations in other domains.

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l p{0.45\textwidth}}
        \toprule
        % \multirow{2}{*}[-1em]{Type} & 
        - According to the {\bf American Library Association}, this makes\dots \\\cline{2-2}
        % & 
        - \dots tasked with drafing a {\bf European Charter of Human Rights},\dots\\
        \midrule
        % \multirow{2}{*}[-0.5em]{Lexicality} & 
        - {\bf The LM engines} were successfully test-fired and restarted, \dots. \\\cline{2-2}
        % & 
        - {\bf Steam turbines} were extensively applied\dots\\
        \midrule
        %\multirow{2}{*}[-1em]{Syntax} & 
        - \dots primarily accomplished through the {\bf ductile stretching and thinning}.\\\cline{2-2}
         % & 
        - \dots directly derived from {\bf the homogeneity or symmetry of space}\dots\\
        \bottomrule
    \end{tabular}%
    }
    \caption{Most similar phrase pairs from disjoint sets of documents. Bold print is the phrase, and non-bold is its context.}
    \label{tab:phrase}
\end{table}

\paragraph{Phrase representations.}
Since \qashort\ models encode all answer candidates into the same space, we expect similar answer candidates to have high inner products with one another.
Table~\ref{tab:phrase} shows pairs of answer candidates that come from different documents in SQuAD, but that have similar encodings (high inner product).
We observe that phrase representations learned through the \qashort\ task capture different interesting characteristics of the phrases.
In all three rows, we can see that the phrase pairs seem to fit into natural categories: national, or multi-national organizational constructs; mechanical engines; and mechanical properties, respectively. 
This suggests that the model has learned interesting typing information above the word level. 
The second and third rows also indicate that the model has learned a rich representation of context. 
This is particularly obvious in the third row where the two phrases are lexically dissimilar, but preceded by the similar contexts {\it `primarily accomplished through'} and {\it `directly derived from'}.
We believe that this analysis, while not complete, points toward exciting future lines of work in learning highly contextualized phrase representations through question answering.

% In the first row, the phrases use distinct words but both refer to national or multi-national organizational constructs. This indicates that ultinatconstructs which indicates that the representations capture the type of the named entity.
% In the second row, we see {\it lexically} and {\it syntactically} similar phrases, where not only `The LM engines' and `Steam turbines' are similar words, but also they are followed by verb--adverb--passive structure.
% In the third row, we now see lexically different but syntactically similar phrases.
% While the meaning of the two phrases are very different, they follow the same structure of adjective--noun-conjunction--noun. Furthermore, the previous surrounding words follow the structure of adverb--passive--proposition. 


\paragraph{Scalability.}
\qashort~can also gain massive execution time speedups once the documents are pre-encoded: in our simple benchmark on a consumer-grade CPU and NumPy (for LSTM+SA model, 1024D vectors), one can easily perform exact search over 1 million document words per second.
BiDAF~\cite{seo2016bidirectional}, an open-sourced and relatively light QA model reaching 77.5\% F1 (66.5\% EM), can process less than 1k document words per second with an equivalent computing power (after pre-encoding the document as much as possible), which is more than 1,000x slower.\footnote{The difference will be even higher with a dedicated similarity search package such as Faiss~\cite{faiss} or approximate search (Section~\ref{sec:problem}).}

It is also important to consider the memory cost for storing a vector representation of each of the answer candidates.
We train an independent single-layer perceptron classifier that predicts whether the phrase encoding is likely to be a good one.
By varying a threshold on the score assigned by this classifier, we can filter answer candidates prior to storage.
Figure~\ref{fig:compression} illustrates the trade-off between accuracy and memory (measured in mean number of vectors per document word) resulting from this filtering procedure for the LSTM+SA model.
We observe that 1.3 vectors (candidates) per word on average reaches $> 98\%$ of the model's F1 accuracy. This is equivalent to 5.2 KB per word with 1024D (4 KB) float vectors, or around 15 TB for the entire English Wikipedia (3 billion words).
Future work will also involve creating a better classifier (i.e. improving the trade-off curve in Figure~\ref{fig:compression}) for determining which phrase vectors to store.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/f1_vs_nvpw.pdf}
    \caption{F1 score versus number of vectors per word for LSTM+SA. Answer candidates have been filtered with varying threshold on an independent classifier learned on the candidate representations.}
    \label{fig:compression}
\end{figure}





==> EMNLP 2018 PIQA/06-conclusion.tex <==
We introduced \QA\ (\qashort), a new variant of the extractive question answering task that requires documents and question encoded completely independently and that they only interact each other via inner product.
We argued that building a question-agnostic document encoder for question answering should be an important consideration for those in the QA community with the research goal of learning a model that reads and comprehends documents.
Furthermore, the imposed constraint of the task implies a sublinear scalability benefit. 
% We analyzed that one of the main challenges of this task is to produce multiple representations for each answer candidate in the document, and we proposed an effective technique called \emph{pivoting} that improves the baselines by 10\% in PI-SQuAD.
Given that SQuAD models have recently outperformed humans,
\qashort\ formulation motivates a new challenge for which we hope that the community's effort gradually closes the gap between our constrained baselines and the unconstrained models.

% We have presented initial experiments in this setting, and have proposed a novel approach that improves performance over LSTM- and self-attention-based baselines by $10\%$ in F1. 
% While we have only investigated simple word based triggers and pivots, \ourapproach~could be extended to arbitrarily complex trigger-pivot functions. 
% We plan to investigate a family of pivot features that relate to multi-word phrases, and capture richer information.

% Finally, \citet{joshi2017triviaqa} recently proposed TriviaQA which pairs each question with a few documents of evidence text, rather than the paragraphs in \squad. On the face of it, this seems to be a more natural fit for our \QA~formalism but we focused on \squad~because we were keen to examine the idea of \QA\ and many `correct' answer spans in TriviaQA do not occur in a context that supports the answer. In future work, we will investigate methods of dealing with this ambiguity.


% Present a new perspective on question answering.
\subsection*{Acknowledgments}
This research was supported by ONR (N00014-18-1-2826), NSF (IIS 1616112), Allen Distinguished Investigator Award, and gifts from Google, Allen Institute for AI, Amazon, and Bloomberg. We  thank the anonymous reviewers for their helpful comments.

